Crossing Number is NP-hard for Constant Path-width (and Tree-width)

The crossing number of a graph is the minimum number of edge crossings that a graph can have when drawn in the plane. Determining this number, known as the Crossing Number problem, is a celebrated problem in combinatorial optimization. It has been known to be NP-complete since the 1980s, and already showing its fixed-parameter tractability when parameterized by the vertex cover number required fairly involved techniques. In this paper, we prove that computing the crossing number exactly remains NP-hard even for graphs of path-width 12 (and as a result, for simple graphs of path-width 13 and tree-width 9). These results highlight that, although both path- and tree-decompositions have been highly successful tools in many graph algorithm scenarios, general crossing number computation is unlikely (under P $\neq$ NP) to be successfully tackled using graph decompositions of bounded width -- a question that had remained a 'tantalizing open problem' [S. Cabello, Hardness of Approximation for Crossing Number, 2013] till now.

==> frame.tex <==
\begin{figure}[h!]
\hspace*{-5ex}% \vspace*{-8ex}

% some special styles/colors....
%\tikzstyle{uweight}=[thick,dotted]
\tikzstyle{uweight}=[very thin, decorate,decoration={zigzag,segment length=3pt,amplitude=0.4}]
%\def\blackpart{}
\def\blackpart{!75!black}
\tikzstyle{framebars}=[brown!50!black,ultra thick]
\tikzstyle{framebars2}=[brown!50!black,ultra thick]
\tikzstyle{varibars}=[black,thick]
\def\tikzonevar#1#2#3{%
  % #1 the x-coordinate,  #2 the height of ladders,  #3 optional suffix of all defined vertices
  \tikzstyle{every node}=[draw, color=red\blackpart, shape=circle, inner sep=0.8pt, fill=red\blackpart]
  \tikzstyle{every path}=[draw, color=red\blackpart]
  % red inner vertices left: (l0)..(l#2), right: (r0)..(r#2)
  \draw[thick] (#1+0.5,1) --++(1,1) node (r0#3){} --++(0,#2) node (r#2#3){} --++(-1,1);
  \draw[uweight,semithick] (#1+0.5,1) --(r0#3) (r#2#3) --++(-1,1);
  \draw[uweight,semithick] (r0#3) --(r#2#3);
  \draw[uweight, semithick] (#1-0.5,1) --++(-1,1) node (l0#3){} --++(0,#2) node (l#2#3){} --++(1,1);
  \draw[thick] (#1-0.5,1) --(l0#3) (l#2#3) --++(1,1);
  \draw[uweight,semithick] (l0#3) --(l#2#3);
  \foreach \xx in {2,3,...,#2} { \tikzmath{integer \x; \x = \xx-1;}
    \node (r\x#3) at (#1+1.5,\x+2) {};  \node (l\x#3) at (#1-1.5,\x+2) {};
  }
  \tikzstyle{every node}=[draw, color=blue\blackpart, shape=circle, inner sep=0.8pt, fill=blue\blackpart]
  \tikzstyle{every path}=[draw, color=blue\blackpart]
  % blue side vertices left: (ll1)..(ll#2), right: (rr1)..(rr#2)
  \draw[thick] (#1+2,1)--(#1+2,#2+3) (#1-2,1)--(#1-2,#2+3);
  \draw[uweight,semithick] (#1+2,1)--(#1+2,#2+3) (#1-2,1)--(#1-2,#2+3);
  \foreach \x in {1,2,...,#2} {
    \node (rr\x#3) at (#1+2,\x+1.5) {};  \node (ll\x#3) at (#1-2,\x+1.5) {};
    \draw (ll\x#3)--++(1,0) (rr\x#3)--++(-1,0);
    %\draw (#1-2,#2+3)--++ (1,-1) (#1-2,1)--++ (1,1) (#1+2,#2+3)--++ (-1,-1) (#1+2,1)--++ (-1,1);
  }
	\tikzstyle{every node}=[draw, varibars, shape=circle, inner sep=1.1pt, fill]
	\tikzstyle{every path}=[draw, framebars]
	\draw (#1,0) node{} --++(2,1) node{} (#1,0) node{} --++(-2,1) node{} (#1+1,2) --++(-2,0);
	\draw (#1,0) node{} --++(0.5,1) node{} --++(-0.5,1) node{} --++(-0.5,-1) node{} -- cycle;
	\draw (#1,#2+4) node{} --++(2,-1) node{} (#1,#2+4) node{} --++(-2,-1) node{} (#1+1,#2+2) --++(-2,0);
	\draw (#1,#2+4) node{} --++(0.5,-1) node{} --++(-0.5,-1) node{} --++(-0.5,1) node{} -- cycle;

  \tikzstyle{every node}=[draw, varibars, shape=circle, inner sep=1.1pt, fill]
  \tikzstyle{every path}=[draw, varibars]
  % black gadget vertices left: (bd),(b1)..(b#2),(bu), right: (cd),(c1)..(c#2),(cu)
  \draw (#1+1,2) node (cd#3) {} (#1-1,2) node (bd#3) {};
  \draw (#1+1,2)--(#1+1,#2+2) (#1-1,2)--(#1-1,#2+2);
  \draw (#1+1,#2+2) node (cu#3) {} (#1-1,#2+2) node (bu#3) {};
  
  \tikzstyle{every node}=[draw, color=black, shape=circle, inner sep=1pt, fill=black]
  \foreach \x in {1,2,...,#2} {
    \node (c\x#3) at (#1+1,\x+1.5) {};  \node (b\x#3) at (#1-1,\x+1.5) {};
  }
}
% fragments of the clause paths
\def\slightup{--++(1.25,0) --++(1.5,0.5) -- ++(0.75,0) --++(0.5,0.5) --++(1,0)}
\def\jumponeup{--++(0.5,0) --++(1.5,1.5) -- ++(1.5,0) --++(0.5,0.5) --++(1,0)}
\def\slightupend{--++(0.5,0.5) --++(2.5,0) --++(1,0.5) --++(1.75,0)}
\def\jumponeupend{--++(0.5,0) --++(1.5,1.5) -- ++(1.5,0) --++(0.75,0)}

\begin{tikzpicture}[scale=0.5]\small
\def\ww{21}\def\hh{8}\def\hho{4}
\tikzstyle{every node}=[draw, varibars, shape=circle, inner sep=1.2pt, fill]
\tikzstyle{every path}=[draw, framebars, rounded corners=3pt]
\draw (0,0)--(-0.3,-0)--(-0.3,\hh)--(0,\hh) (\ww,0)--(\ww.3,-0)--(\ww.3,\hh)--(\ww,\hh);
\draw (0,0)--(0,-0.3)--(\ww,-0.3)--(\ww,0)
(0,\hh)--(0,\hh.3)--(\ww,\hh.3)--(\ww,\hh);
\draw (0,-0.03) node{} --(\ww,-0.03) node{} --(\ww,\hh.03) node{} --(0,\hh.03) node{} -- cycle;
% \draw (-0.3,-0.3)--(\ww.3,-0.3)--(\ww.3,\hh.3)--(-0.3,\hh.3)-- cycle;


\foreach \v/\a in {3/a,8/b,18/c} {
	\tikzonevar{\v}{\hho}{\a}
}

\end{tikzpicture}

\caption{A schematic picture of .....................
frame -- very thick brown, variable gadgets -- black and blue, bundle gadgets -- red, clauses -- green edges ...............
}\label{fig:redu-all}
% \vspace*{28ex}
\end{figure}

==> var_base.tex <==
\begin{figure}[h!]
\hspace*{-5ex}% \vspace*{-8ex}

% some special styles/colors....
%\tikzstyle{uweight}=[thick,dotted]
\tikzstyle{uweight}=[very thin, decorate,decoration={zigzag,segment length=3pt,amplitude=0.4}]
%\def\blackpart{}
\def\blackpart{!75!black}
\tikzstyle{framebars}=[brown!50!black,ultra thick]
\tikzstyle{framebars2}=[brown!50!black,ultra thick]
\tikzstyle{varibars}=[black,thick]
\def\tikzonevar#1#2#3{%
  % #1 the x-coordinate,  #2 the height of ladders,  #3 optional suffix of all defined vertices
  \tikzstyle{every node}=[draw, color=red\blackpart, shape=circle, inner sep=0.8pt, fill=red\blackpart]
  \tikzstyle{every path}=[draw, color=red\blackpart]
  % red inner vertices left: (l0)..(l#2), right: (r0)..(r#2)
  \draw[thick] (#1+0.5,1) --++(1,1) node (r0#3){} --++(0,#2) node (r#2#3){} --++(-1,1);
  \draw[uweight,semithick] (#1+0.5,1) --(r0#3) (r#2#3) --++(-1,1);
  \draw[uweight,semithick] (r0#3) --(r#2#3);
  \draw[uweight, semithick] (#1-0.5,1) --++(-1,1) node (l0#3){} --++(0,#2) node (l#2#3){} --++(1,1);
  \draw[thick] (#1-0.5,1) --(l0#3) (l#2#3) --++(1,1);
  \draw[uweight,semithick] (l0#3) --(l#2#3);
  \foreach \xx in {2,3,...,#2} { \tikzmath{integer \x; \x = \xx-1;}
    \node (r\x#3) at (#1+1.5,\x+2) {};  \node (l\x#3) at (#1-1.5,\x+2) {};
  }
  \tikzstyle{every node}=[draw, color=blue\blackpart, shape=circle, inner sep=0.8pt, fill=blue\blackpart]
  \tikzstyle{every path}=[draw, color=blue\blackpart]
  % blue side vertices left: (ll1)..(ll#2), right: (rr1)..(rr#2)
  \draw[thick] (#1+2,1)--(#1+2,#2+3) (#1-2,1)--(#1-2,#2+3);
  \draw[uweight,semithick] (#1+2,1)--(#1+2,#2+3) (#1-2,1)--(#1-2,#2+3);
  \foreach \x in {1,2,...,#2} {
    \node (rr\x#3) at (#1+2,\x+1.5) {};  \node (ll\x#3) at (#1-2,\x+1.5) {};
    \draw (ll\x#3)--++(1,0) (rr\x#3)--++(-1,0);
    %\draw (#1-2,#2+3)--++ (1,-1) (#1-2,1)--++ (1,1) (#1+2,#2+3)--++ (-1,-1) (#1+2,1)--++ (-1,1);
  }
	\tikzstyle{every node}=[draw, varibars, shape=circle, inner sep=1.1pt, fill]
	\tikzstyle{every path}=[draw, framebars]
	\draw (#1,0) node{} --++(2,1) node{} (#1,0) node{} --++(-2,1) node{} (#1+1,2) --++(-2,0);
	\draw (#1,0) node{} --++(0.5,1) node{} --++(-0.5,1) node{} --++(-0.5,-1) node{} -- cycle;
	\draw (#1,#2+4) node{} --++(2,-1) node{} (#1,#2+4) node{} --++(-2,-1) node{} (#1+1,#2+2) --++(-2,0);
	\draw (#1,#2+4) node{} --++(0.5,-1) node{} --++(-0.5,-1) node{} --++(-0.5,1) node{} -- cycle;

  \tikzstyle{every node}=[draw, varibars, shape=circle, inner sep=1.1pt, fill]
  \tikzstyle{every path}=[draw, varibars]
  % black gadget vertices left: (bd),(b1)..(b#2),(bu), right: (cd),(c1)..(c#2),(cu)
  \draw (#1+1,2) node (cd#3) {} (#1-1,2) node (bd#3) {};
  \draw (#1+1,2)--(#1+1,#2+2) (#1-1,2)--(#1-1,#2+2);
  \draw (#1+1,#2+2) node (cu#3) {} (#1-1,#2+2) node (bu#3) {};
  
  \tikzstyle{every node}=[draw, color=black, shape=circle, inner sep=1pt, fill=black]
  \foreach \x in {1,2,...,#2} {
    \node (c\x#3) at (#1+1,\x+1.5) {};  \node (b\x#3) at (#1-1,\x+1.5) {};
  }
}

\begin{tikzpicture}[scale=0.5]\small
\def\ww{15}\def\hh{10}\def\hho{1}

\foreach \v/\a in {3/a} {
	\tikzonevar{\v}{0}{\a}
}
\tikzstyle{every node}=[draw, color=black, shape=circle, inner sep=0.8pt, fill=black]
\tikzstyle{every path}=[draw]

%\draw[very thick, loosely dotted, gray] (b1a)++(1,1.5) -- ++(0,2);

\end{tikzpicture}

\caption{A schematic picture of variable gadget
}\label{fig:variable}
% \vspace*{28ex}
\end{figure}

==> variable.tex <==
\begin{figure}[h!]
\hspace*{-5ex}% \vspace*{-8ex}

% some special styles/colors....
%\tikzstyle{uweight}=[thick,dotted]
\tikzstyle{uweight}=[very thin, decorate,decoration={zigzag,segment length=3pt,amplitude=0.4}]
%\def\blackpart{}
\def\blackpart{!75!black}
\tikzstyle{framebars}=[brown!50!black,ultra thick]
\tikzstyle{framebars2}=[brown!50!black,ultra thick]
\tikzstyle{varibars}=[black,thick]
\def\tikzonevar#1#2#3{%
  % #1 the x-coordinate,  #2 the height of ladders,  #3 optional suffix of all defined vertices
  \tikzstyle{every node}=[draw, color=red\blackpart, shape=circle, inner sep=0.8pt, fill=red\blackpart]
  \tikzstyle{every path}=[draw, color=red\blackpart]
  % red inner vertices left: (l0)..(l#2), right: (r0)..(r#2)
  \draw[thick] (#1+0.5,1) --++(1,1) node (r0#3){} --++(0,#2) node (r#2#3){} --++(-1,1);
  \draw[uweight,semithick] (#1+0.5,1) --(r0#3) (r#2#3) --++(-1,1);
  \draw[uweight,semithick] (r0#3) --(r#2#3);
  \draw[uweight, semithick] (#1-0.5,1) --++(-1,1) node (l0#3){} --++(0,#2) node (l#2#3){} --++(1,1);
  \draw[thick] (#1-0.5,1) --(l0#3) (l#2#3) --++(1,1);
  \draw[uweight,semithick] (l0#3) --(l#2#3);
  \foreach \xx in {2,3,...,#2} { \tikzmath{integer \x; \x = \xx-1;}
    \node (r\x#3) at (#1+1.5,\x+2) {};  \node (l\x#3) at (#1-1.5,\x+2) {};
  }
  \tikzstyle{every node}=[draw, color=blue\blackpart, shape=circle, inner sep=0.8pt, fill=blue\blackpart]
  \tikzstyle{every path}=[draw, color=blue\blackpart]
  % blue side vertices left: (ll1)..(ll#2), right: (rr1)..(rr#2)
  \draw[thick] (#1+2,1)--(#1+2,#2+3) (#1-2,1)--(#1-2,#2+3);
  \draw[uweight,semithick] (#1+2,1)--(#1+2,#2+3) (#1-2,1)--(#1-2,#2+3);
  \foreach \x in {1,2,...,#2} {
    \node (rr\x#3) at (#1+2,\x+1.5) {};  \node (ll\x#3) at (#1-2,\x+1.5) {};
    \draw (ll\x#3)--++(1,0) (rr\x#3)--++(-1,0);
    %\draw (#1-2,#2+3)--++ (1,-1) (#1-2,1)--++ (1,1) (#1+2,#2+3)--++ (-1,-1) (#1+2,1)--++ (-1,1);
  }
	\tikzstyle{every node}=[draw, varibars, shape=circle, inner sep=1.1pt, fill]
	\tikzstyle{every path}=[draw, framebars]
	\draw (#1,0) node{} --++(2,1) node{} (#1,0) node{} --++(-2,1) node{} (#1+1,2) --++(-2,0);
	\draw (#1,0) node{} --++(0.5,1) node{} --++(-0.5,1) node{} --++(-0.5,-1) node{} -- cycle;
	\draw (#1,#2+4) node{} --++(2,-1) node{} (#1,#2+4) node{} --++(-2,-1) node{} (#1+1,#2+2) --++(-2,0);
	\draw (#1,#2+4) node{} --++(0.5,-1) node{} --++(-0.5,-1) node{} --++(-0.5,1) node{} -- cycle;

  \tikzstyle{every node}=[draw, varibars, shape=circle, inner sep=1.1pt, fill]
  \tikzstyle{every path}=[draw, varibars]
  % black gadget vertices left: (bd),(b1)..(b#2),(bu), right: (cd),(c1)..(c#2),(cu)
  \draw (#1+1,2) node (cd#3) {} (#1-1,2) node (bd#3) {};
  \draw (#1+1,2)--(#1+1,#2+2) (#1-1,2)--(#1-1,#2+2);
  \draw (#1+1,#2+2) node (cu#3) {} (#1-1,#2+2) node (bu#3) {};
  
  \tikzstyle{every node}=[draw, color=black, shape=circle, inner sep=1pt, fill=black]
  \foreach \x in {1,2,...,#2} {
    \node (c\x#3) at (#1+1,\x+1.5) {};  \node (b\x#3) at (#1-1,\x+1.5) {};
  }
}

\begin{tikzpicture}[scale=0.5]\small
\def\ww{15}\def\hh{10}\def\hho{4}

\foreach \v/\a in {3/a} {
	\tikzonevar{\v}{\hho}{\a}
}
\tikzstyle{every node}=[draw, color=black, shape=circle, inner sep=0.8pt, fill=black]
\tikzstyle{every path}=[draw]

%\draw[very thick, loosely dotted, gray] (b1a)++(1,1.5) -- ++(0,2);

\end{tikzpicture}

\caption{A schematic picture of variable gadget
}\label{fig:variable}
% \vspace*{28ex}
\end{figure}
